Weak Scale Leptogenesis, R-symmetry, and a Displaced Higgs

We present a supersymmetric model of leptogenesis in which the right-handed neutrinos have weak scale masses and O(10-2-10-3) yukawa couplings. The model employs an R-symmetry at the weak scale that forces neutrino masses to be proportional to the gravitino mass. We predict that the lightest right-handed neutrino decays to a displaced Higgs and neutrino and that the NLSP is long-lived on collider scales. These could be striking signatures at the LHC if, for instance, the right-handed neutrino is produced in a cascade decay.

==> Submission copy/author_list.tex <==
% remove these 3 lines before journal submittal.
% end removal before journal submittal
%
\affiliation{Massachusetts Institute of Technology, Cambridge, Massachusetts 02139}
\affiliation{Houghton College, Houghton, New York 00000}
%
\author{Keith Rehermann} \affiliation{Massachusetts Institute of Technology, Cambridge, Massachusetts 02139} 
\author{Christopher M.~Wells} \affiliation{Houghton College, Houghton, New York 14744}
%
% visitor_addresses.tex                        2 August 2011
%  available symbols are:
%  $\ast, \dag, \ddag, \S, \P, $\|$, $\ast\ast$, \dag\dag, \ddag\ddag ,\#
%
%
\vskip 0.25cm


==> Submission copy/short_cuts.tex <==
\DeclareGraphicsRule{.tif}{png}{.png}{`convert #1 `dirname #1`/`basename #1 .tif`.png}



\def\lsim{\mathrel{\rlap{\lower4pt\hbox{\hskip1pt$\sim$}}
    \raise1pt\hbox{$<$}}}
\def\gsim{\mathrel{\rlap{\lower4pt\hbox{\hskip1pt$\sim$}}
    \raise1pt\hbox{$>$}}} 
\newcommand{\vev}[1]{ \left\langle {#1} \right\rangle }
\newcommand{\bra}[1]{ \langle {#1} | }
\newcommand{\ket}[1]{ | {#1} \rangle }

%% Scales and Units
\newcommand{\ev}{ {\rm eV} }
\newcommand{\kev}{{\rm keV}}
\newcommand{\mev}{{\rm MeV}}
\newcommand{\gev}{{\rm GeV}}
\newcommand{\tev}{{\rm TeV}}
\newcommand{\mpl}{$M_{Pl}$}
\newcommand{\mw}{$M_{W}$}
\newcommand{\mz}{$M_{Z}$}

\newcommand{\hc}[1]{#1^{\dagger}}

\newcommand{\Ft}{F_{T}}
\newcommand{\Zparity}{$\mathbb{Z}_2$}
\newcommand{\BLambda}{\boldsymbol{\lambda}}
\newcommand{\Bgamma}{\boldsymbol{\gamma}}
\newcommand{\be}{\begin{eqnarray}}
\newcommand{\ee}{\end{eqnarray}}
\newcommand{\fslash}{\displaystyle{\not}}

\newcommand{\boldgamma}{\textbf{\scriptsize{$\gamma$}}}
\newcommand{\bolde}{\textbf{\scriptsize{e}}}
\newcommand{\rhat}{\hat{\vec{r}}}
\newcommand{\phat}{\hat{\vec{p}}}

%% organzition for parenthesis
\newcommand{\parfrac}[2]{\left(\frac{#1}{#2}\right)}


%% lowercase cursive
\newenvironment{frcseries}{\fontfamily{frc}\selectfont}{}
\newcommand{\textfrc}[1]{{\frcseries#1}}
\newcommand{\mathfrc}[1]{\text{\textfrc{#1}}}

%\newcommand{\im}{\mathfrc{Im}}
\newcommand{\im}{\mathcal{I}m}

%% neutrinos
\newcommand{\mnu}{m_{\nu}}
\newcommand{\dMnuAtm}{\Delta m^2_{\rm{atm}}}
\newcommand{\dMnuSol}{\Delta m^2_{\rm{\odot}}}

%%
\newcommand{\HubbleAtM}[1]{H|_{T=M_{#1}}}

\newcommand{\nuc}{\nu^c}
\newcommand{\Ynuc}{Y^{\nu^c}}
\newcommand{\Msigma}{M_{\Sigma}}
\newcommand{\SigmaBar}{\overline{\Sigma}}
\newcommand{\order}{\mathcal{O}}
\newcommand{\op}{\mathcal{O}}
\newcommand{\lag}[1]{\mathcal{L_{#1}}}
%\newcommand{\d}[1]{\partial_{#1}}
\newcommand{\Nwidth}{\Gamma_{N_1}}

%% for adding comments
\newcommand{\KR}[1]{{\bf \color{red} (#1 -k)}}

%% mssm
\newcommand{\tanb}{\tan\beta}
\newcommand{\ssoftmass}[1]{\tilde{m}^2_{#1}}
\newcommand{\bino}{\tilde{B}}
\newcommand{\snu}{\tilde{\nu}}
\newcommand{\stauc}{\tilde{\tau}^c}
\newcommand{\stopc}{\tilde{t}^c}


%% new states
\newcommand{\mpsi}{m_{\psi}}
\newcommand{\Mpsi}{M_{\psi}}
\newcommand{\mphi}{m_{\phi}}
\newcommand{\Mphi}{M_{\phi}}


%% superspace
\newcommand{\dFtheta}{\int d^4 \theta}
\newcommand{\dTtheta}{\int d^2 \theta}
\newcommand{\Dalpha}[1]{D#1{\alpha}}
\newcommand{\sPot}{\mathcal{W}}
\newcommand{\mgrav}{m_{3/2}}

%% ref shortcuts
\newcommand{\eqn}[1]{Eq.\,(\ref{#1})} 
\newcommand{\tab}[1]{Table\,\ref{#1}} 
\newcommand{\fig}[1]{Fig.\,\ref{#1}}
\newcommand{\myref}[1]{Ref.\,\cite{#1}}
